Asteroseismic modelling of solar-type stars: internal systematics from input physics and surface correction methods

Asteroseismic forward modelling techniques are being used to determine fundamental properties (e.g. mass, radius, and age) of solar-type stars. The need to take into account all possible sources of error is of paramount importance towards a robust determination of stellar properties. We present a study of 34 solar-type stars for which high signal-to-noise asteroseismic data is available from multi-year Kepler photometry. We explore the internal systematics on the stellar properties, that is, associated with the uncertainty in the input physics used to construct the stellar models. In particular, we explore the systematics arising from: (i) the inclusion of the diffusion of helium and heavy elements; and (ii) the uncertainty in solar metallicity mixture. We also assess the systematics arising from (iii) different surface correction methods used in optimisation/fitting procedures. The systematics arising from comparing results of models with and without diffusion are found to be 0.5%, 0.8%, 2.1%, and 16% in mean density, radius, mass, and age, respectively. The internal systematics in age are significantly larger than the statistical uncertainties. We find the internal systematics resulting from the uncertainty in solar metallicity mixture to be 0.7% in mean density, 0.5% in radius, 1.4% in mass, and 6.7% in age. The surface correction method by Sonoi et al. and Ball & Gizon's two-term correction produce the lowest internal systematics among the different correction methods, namely, ~1%, ~1%, ~2%, and ~8% in mean density, radius, mass, and age, respectively. Stellar masses obtained using the surface correction methods by Kjeldsen et al. and Ball & Gizon's one-term correction are systematically higher than those obtained using frequency ratios.

==> mybib <==
@ARTICLE{Monteiro,
   author = {{Monteiro}, M.~J.~P.~F.~G. and {Christensen-Dalsgaard}, J. and 
	{Thompson}, M.~J.},
    title = "{Seismic properties of the Sun's superadiabatic layer. I. Theoretical modelling and parametrization of the uncertainties.}",
  journal = {A \& A},
 keywords = {SUN: INTERIOR, SUN: OSCILLATIONS, CONVECTION},
     year = 1996,
    month = mar,
   volume = 307,
    pages = {624-634},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...307..624M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Thomps,
   author = {{Christensen-Dalsgaard}, J. and {Monteiro}, M.~J.~P.~F.~G. and 
	{Rempel}, M. and {Thompson}, M.~J.},
    title = "{A more realistic representation of overshoot at the base of the solar convective envelope as seen by helioseismology}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1102.0235},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, convection, Sun: helioseismology, Sun: interior, stars: interiors},
     year = 2011,
    month = jun,
   volume = 414,
    pages = {1158-1174},
      doi = {10.1111/j.1365-2966.2011.18460.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.1158C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Perryman2014,
   author = {{Perryman}, M.},
    title = "{The Exoplanet Handbook, Cambridge, UK: Cambridge University Press}",
booktitle = {The Exoplanet Handbook, by Michael Perryman, Cambridge, UK: Cambridge University Press, 2014},
     year = 2014,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2014exha.book.....P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Gregory,
   author = {{Gregory}, P.~C.},
    title = "{Bayesian Logical Data Analysis for the Physical Sciences: A Comparative Approach with `Mathematica' Support}",
booktitle = {Bayesian Logical Data Analysis for the Physical Sciences: A Comparative Approach with `Mathematica' Support.~Edited by P.~C.~Gregory.~ISBN 0 521 84150 X (hardback); QA279.5.G74 2005 519.5'42 -- dc22; 200445930.~Published by Cambridge University Press, Cambridge, UK, 2005.},
     year = 2005,
    month = apr,
publisher = {Cambridge University Press},
   adsurl = {http://adsabs.harvard.edu/abs/2005blda.book.....G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Trampedach,
   author = {{Trampedach}, R. and {Stein}, R.~F.},
    title = "{The Mass Mixing Length in Convective Stellar Envelopes}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1102.1102},
 primaryClass = "astro-ph.SR",
 keywords = {convection, methods: numerical, stars: late-type},
     year = 2011,
    month = apr,
   volume = 731,
      eid = {78},
    pages = {78},
      doi = {10.1088/0004-637X/731/2/78},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...731...78T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goldreich,
   author = {{Goldreich}, P. and {Murray}, N. and {Willette}, G. and {Kumar}, P.
	},
    title = "{Implications of solar p-mode frequency shifts}",
  journal = {ApJ},
 keywords = {Frequency Shift, Magnetohydrodynamics, Solar Magnetic Field, Solar Oscillations, Brightness Distribution, Chromosphere, Entropy, Frequency Distribution, Magnetic Disturbances},
     year = 1991,
    month = apr,
   volume = 370,
    pages = {752-762},
      doi = {10.1086/169858},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...370..752G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Deheuvels2014,
   author = {{Deheuvels}, S. and {Do{\u g}an}, G. and {Goupil}, M.~J. and 
	{Appourchaux}, T. and {Benomar}, O. and {Bruntt}, H. and {Campante}, T.~L. and 
	{Casagrande}, L. and {Ceillier}, T. and {Davies}, G.~R. and 
	{De Cat}, P. and {Fu}, J.~N. and {Garc{\'{\i}}a}, R.~A. and 
	{Lobel}, A. and {Mosser}, B. and {Reese}, D.~R. and {Regulo}, C. and 
	{Schou}, J. and {Stahn}, T. and {Thygesen}, A.~O. and {Yang}, X.~H. and 
	{Chaplin}, W.~J. and {Christensen-Dalsgaard}, J. and {Eggenberger}, P. and 
	{Gizon}, L. and {Mathis}, S. and {Molenda-{\.Z}akowicz}, J. and 
	{Pinsonneault}, M.},
    title = "{Seismic constraints on the radial dependence of the internal rotation profiles of six Kepler subgiants and young red giants}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1401.3096},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: rotation, stars: interiors, stars: evolution},
     year = 2014,
    month = apr,
   volume = 564,
      eid = {A27},
    pages = {A27},
      doi = {10.1051/0004-6361/201322779},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...564A..27D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@Inbook{Gough1990,
author="Gough, Douglas",
editor="Osaki, Y.
and Shibahashi, H.",
title="Comments on helioseismic inference, in Progress of Seismology of the Sun and Stars",
year="1990",
editors="Osaki Y. and Shibahashi H.",
pages="Lecture Notes in Physics, Vol 367, 283",
publisher="Springer Berlin Heidelberg",
isbn="978-3-540-46645-1",
doi="10.1007/3-540-53091-6_93"
}


@ARTICLE{Reese,
   author = {{Lund}, M.~N. and {Reese}, D.~R.},
    title = "{Asteroseismic Stellar Modelling with AIMS}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1711.01896},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
     year = 2017,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv171101896L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Piau,
   author = {{Piau}, L. and {Kervella}, P. and {Dib}, S. and {Hauschildt}, P.
	},
    title = "{Surface convection and red-giant radius measurements}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1010.3649},
 primaryClass = "astro-ph.SR",
 keywords = {stars: low-mass, convection, stars: evolution, asteroseismology},
     year = 2011,
    month = feb,
   volume = 526,
      eid = {A100},
    pages = {A100},
      doi = {10.1051/0004-6361/201014442},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...526A.100P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Deheuvels,
   author = {{Deheuvels}, S. and {Michel}, E.},
    title = "{Constraints on the structure of the core of subgiants via mixed modes: the case of HD 49385}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1109.1191},
 primaryClass = "astro-ph.SR",
 keywords = {stars: oscillations, stars: evolution, stars: interiors, stars: individual: HD 49385},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {A91},
    pages = {A91},
      doi = {10.1051/0004-6361/201117232},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...535A..91D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Silva,
   author = {{Silva Aguirre}, V. and {Ballot}, J. and {Serenelli}, A.~M. and 
	{Weiss}, A.},
    title = "{Constraining mixing processes in stellar cores using asteroseismology. Impact of semiconvection in low-mass stars}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1102.0779},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, convection, asteroseismology, stars: oscillations},
     year = 2011,
    month = may,
   volume = 529,
      eid = {A63},
    pages = {A63},
      doi = {10.1051/0004-6361/201015847},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529A..63S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Thoul,
   author = {{Thoul}, A.~A. and {Bahcall}, J.~N. and {Loeb}, A.},
    title = "{Element diffusion in the solar interior}",
  journal = {ApJ},
   eprint = {astro-ph/9304005},
 keywords = {Abundance, Diffusion, Flow Equations, Heavy Elements, Helium, Solar Interior, Stellar Composition, Stellar Models, Computerized Simulation, Stellar Evolution, Subroutines},
     year = 1994,
    month = feb,
   volume = 421,
    pages = {828-842},
      doi = {10.1086/173695},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...421..828T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Turcotte,
   author = {{Turcotte}, S. and {Richer}, J. and {Michaud}, G. and {Iglesias}, C.~A. and 
	{Rogers}, F.~J.},
    title = "{Consistent Solar Evolution Model Including Diffusion and Radiative Acceleration Effects}",
  journal = {ApJ},
 keywords = {DIFFUSION, SUN: ABUNDANCES, SUN: EVOLUTION, SUN: INTERIOR, Diffusion, Sun: Abundances, Sun: Evolution, Sun: Interior},
     year = 1998,
    month = sep,
   volume = 504,
    pages = {539-558},
      doi = {10.1086/306055},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...504..539T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maeder,
   author = {{Maeder}, A. and {Meynet}, G.},
    title = "{The Evolution of Rotating Stars}",
  journal = {Annual Review of Astron and Astrophys},
   eprint = {astro-ph/0004204},
 keywords = {STELLAR ROTATION, STELLAR EVOLUTION, MASS LOSS, MIXING, CHEMICAL ABUNDANCES},
     year = 2000,
   volume = 38,
    pages = {143-190},
      doi = {10.1146/annurev.astro.38.1.143},
   adsurl = {http://adsabs.harvard.edu/abs/2000ARA%26A..38..143M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Grevesse,
   author = {{Grevesse}, N. and {Sauval}, A.~J.},
    title = "{Standard Solar Composition}",
  journal = {Space Science Reviews},
 keywords = {Sun: abundances, Meteorites: abundances, Solar spectroscopy},
     year = 1998,
    month = may,
   volume = 85,
    pages = {161-174},
      doi = {10.1023/A:1005161325181},
   adsurl = {http://adsabs.harvard.edu/abs/1998SSRv...85..161G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rauer1,
   author = {{Rauer}, H. and {Catala}, C. and {Aerts}, C. and {Appourchaux}, T. and 
	{Benz}, W. and {Brandeker}, A. and {Christensen-Dalsgaard}, J. and 
	{Deleuil}, M. and {Gizon}, L. and {Goupil}, M.-J. and {G{\"u}del}, M. and 
	{Janot-Pacheco}, E. and {Mas-Hesse}, M. and {Pagano}, I. and 
	{Piotto}, G. and {Pollacco}, D. and {Santos}, {\.C}. and {Smith}, A. and 
	{Su{\'a}rez}, J.-C. and {Szab{\'o}}, R. and {Udry}, S. and {Adibekyan}, V. and 
	{Alibert}, Y. and {Almenara}, J.-M. and {Amaro-Seoane}, P. and 
	{Eiff}, M.~A.-v. and {Asplund}, M. and {Antonello}, E. and {Barnes}, S. and 
	{Baudin}, F. and {Belkacem}, K. and {Bergemann}, M. and {Bihain}, G. and 
	{Birch}, A.~C. and {Bonfils}, X. and {Boisse}, I. and {Bonomo}, A.~S. and 
	{Borsa}, F. and {Brand{\~a}o}, I.~M. and {Brocato}, E. and {Brun}, S. and 
	{Burleigh}, M. and {Burston}, R. and {Cabrera}, J. and {Cassisi}, S. and 
	{Chaplin}, W. and {Charpinet}, S. and {Chiappini}, C. and {Church}, R.~P. and 
	{Csizmadia}, S. and {Cunha}, M. and {Damasso}, M. and {Davies}, M.~B. and 
	{Deeg}, H.~J. and {D{\'{\i}}az}, R.~F. and {Dreizler}, S. and 
	{Dreyer}, C. and {Eggenberger}, P. and {Ehrenreich}, D. and 
	{Eigm{\"u}ller}, P. and {Erikson}, A. and {Farmer}, R. and {Feltzing}, S. and 
	{de Oliveira Fialho}, F. and {Figueira}, P. and {Forveille}, T. and 
	{Fridlund}, M. and {Garc{\'{\i}}a}, R.~A. and {Giommi}, P. and 
	{Giuffrida}, G. and {Godolt}, M. and {Gomes da Silva}, J. and 
	{Granzer}, T. and {Grenfell}, J.~L. and {Grotsch-Noels}, A. and 
	{G{\"u}nther}, E. and {Haswell}, C.~A. and {Hatzes}, A.~P. and 
	{H{\'e}brard}, G. and {Hekker}, S. and {Helled}, R. and {Heng}, K. and 
	{Jenkins}, J.~M. and {Johansen}, A. and {Khodachenko}, M.~L. and 
	{Kislyakova}, K.~G. and {Kley}, W. and {Kolb}, U. and {Krivova}, N. and 
	{Kupka}, F. and {Lammer}, H. and {Lanza}, A.~F. and {Lebreton}, Y. and 
	{Magrin}, D. and {Marcos-Arenal}, P. and {Marrese}, P.~M. and 
	{Marques}, J.~P. and {Martins}, J. and {Mathis}, S. and {Mathur}, S. and 
	{Messina}, S. and {Miglio}, A. and {Montalban}, J. and {Montalto}, M. and 
	{Monteiro}, M.~J.~P.~F.~G. and {Moradi}, H. and {Moravveji}, E. and 
	{Mordasini}, C. and {Morel}, T. and {Mortier}, A. and {Nascimbeni}, V. and 
	{Nelson}, R.~P. and {Nielsen}, M.~B. and {Noack}, L. and {Norton}, A.~J. and 
	{Ofir}, A. and {Oshagh}, M. and {Ouazzani}, R.-M. and {P{\'a}pics}, P. and 
	{Parro}, V.~C. and {Petit}, P. and {Plez}, B. and {Poretti}, E. and 
	{Quirrenbach}, A. and {Ragazzoni}, R. and {Raimondo}, G. and 
	{Rainer}, M. and {Reese}, D.~R. and {Redmer}, R. and {Reffert}, S. and 
	{Rojas-Ayala}, B. and {Roxburgh}, I.~W. and {Salmon}, S. and 
	{Santerne}, A. and {Schneider}, J. and {Schou}, J. and {Schuh}, S. and 
	{Schunker}, H. and {Silva-Valio}, A. and {Silvotti}, R. and 
	{Skillen}, I. and {Snellen}, I. and {Sohl}, F. and {Sousa}, S.~G. and 
	{Sozzetti}, A. and {Stello}, D. and {Strassmeier}, K.~G. and 
	{{\v S}vanda}, M. and {Szab{\'o}}, G.~M. and {Tkachenko}, A. and 
	{Valencia}, D. and {Van Grootel}, V. and {Vauclair}, S.~D. and 
	{Ventura}, P. and {Wagner}, F.~W. and {Walton}, N.~A. and {Weingrill}, J. and 
	{Werner}, S.~C. and {Wheatley}, P.~J. and {Zwintz}, K.},
    title = "{The PLATO 2.0 mission}",
  journal = {Experimental Astronomy},
archivePrefix = "arXiv",
   eprint = {1310.0696},
 primaryClass = "astro-ph.EP",
 keywords = {Exoplanets, Asteroseismology, Transit survey, Stellar science, Exoplanetary science},
     year = 2014,
    month = nov,
   volume = 38,
    pages = {249-330},
      doi = {10.1007/s10686-014-9383-4},
   adsurl = {http://adsabs.harvard.edu/abs/2014ExA....38..249R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kawaler,
   author = {{Silva Aguirre}, V. and {Basu}, S. and {Brand{\~a}o}, I.~M. and 
	{Christensen-Dalsgaard}, J. and {Deheuvels}, S. and {Do{\u g}an}, G. and 
	{Metcalfe}, T.~S. and {Serenelli}, A.~M. and {Ballot}, J. and 
	{Chaplin}, W.~J. and {Cunha}, M.~S. and {Weiss}, A. and {Appourchaux}, T. and 
	{Casagrande}, L. and {Cassisi}, S. and {Creevey}, O.~L. and 
	{Garc{\'{\i}}a}, R.~A. and {Lebreton}, Y. and {Noels}, A. and 
	{Sousa}, S.~G. and {Stello}, D. and {White}, T.~R. and {Kawaler}, S.~D. and 
	{Kjeldsen}, H.},
    title = "{Stellar Ages and Convective Cores in Field Main-sequence Stars: First Asteroseismic Application to Two Kepler Targets}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1304.2772},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: fundamental parameters, stars: interiors, stars: oscillations },
     year = 2013,
    month = jun,
   volume = 769,
      eid = {141},
    pages = {141},
      doi = {10.1088/0004-637X/769/2/141},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...769..141S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Still,
   author = {{Metcalfe}, T.~S. and {Chaplin}, W.~J. and {Appourchaux}, T. and 
	{Garc{\'{\i}}a}, R.~A. and {Basu}, S. and {Brand{\~a}o}, I. and 
	{Creevey}, O.~L. and {Deheuvels}, S. and {Do{\v g}an}, G. and 
	{Eggenberger}, P. and {Karoff}, C. and {Miglio}, A. and {Stello}, D. and 
	{Y{\i}ld{\i}z}, M. and {{\c C}elik}, Z. and {Antia}, H.~M. and 
	{Benomar}, O. and {Howe}, R. and {R{\'e}gulo}, C. and {Salabert}, D. and 
	{Stahn}, T. and {Bedding}, T.~R. and {Davies}, G.~R. and {Elsworth}, Y. and 
	{Gizon}, L. and {Hekker}, S. and {Mathur}, S. and {Mosser}, B. and 
	{Bryson}, S.~T. and {Still}, M.~D. and {Christensen-Dalsgaard}, J. and 
	{Gilliland}, R.~L. and {Kawaler}, S.~D. and {Kjeldsen}, H. and 
	{Ibrahim}, K.~A. and {Klaus}, T.~C. and {Li}, J.},
    title = "{Asteroseismology of the Solar Analogs 16 Cyg A and B from Kepler Observations}",
  journal = {APJL},
archivePrefix = "arXiv",
   eprint = {1201.5966},
 primaryClass = "astro-ph.SR",
 keywords = {stars: fundamental parameters, stars: individual: HD 186408 HD 186427, stars: interiors, stars: oscillations, stars: solar-type},
     year = 2012,
    month = mar,
   volume = 748,
      eid = {L10},
    pages = {L10},
      doi = {10.1088/2041-8205/748/1/L10},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748L..10M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Monta,
   author = {{Miglio}, A. and {Montalb{\'a}n}, J.},
    title = "{Constraining fundamental stellar parameters using seismology. Application to {$\alpha$} Centauri AB}",
  journal = {A&A},
   eprint = {astro-ph/0505537},
 keywords = {stars: oscillations, stars: interiors, stars: fundamental parameters, stars: individual: {$\alpha$} Cen},
     year = 2005,
    month = oct,
   volume = 441,
    pages = {615-629},
      doi = {10.1051/0004-6361:20052988},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...441..615M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dav,
   author = {{Davies}, G.~R. and {Silva Aguirre}, V. and {Bedding}, T.~R. and 
	{Handberg}, R. and {Lund}, M.~N. and {Chaplin}, W.~J. and {Huber}, D. and 
	{White}, T.~R. and {Benomar}, O. and {Hekker}, S. and {Basu}, S. and 
	{Campante}, T.~L. and {Christensen-Dalsgaard}, J. and {Elsworth}, Y. and 
	{Karoff}, C. and {Kjeldsen}, H. and {Lundkvist}, M.~S. and {Metcalfe}, T.~S. and 
	{Stello}, D.},
    title = "{Oscillation frequencies for 35 Kepler solar-type planet-hosting stars using Bayesian techniques and machine learning}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1511.02105},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, planets and satellites: fundamental parameters, stars: evolution, stars: fundamental parameters, stars: oscillations, planetary systems},
     year = 2016,
    month = feb,
   volume = 456,
    pages = {2183-2195},
      doi = {10.1093/mnras/stv2593},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.456.2183D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Beno,
   author = {{Benomar}, O. and {Masuda}, K. and {Shibahashi}, H. and {Suto}, Y.
	},
    title = "{Determination of three-dimensional spin-orbit angle with joint analysis of asteroseismology, transit lightcurve, and the Rossiter-McLaughlin effect: Cases of HAT-P-7 and Kepler-25}",
  journal = {PASJ},
archivePrefix = "arXiv",
   eprint = {1407.7332},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: individual (HAT-P-7, KOI-2, KIC 10666592), stars: individual (Kepler-25, KOI-244, KIC 4349452)},
     year = 2014,
    month = oct,
   volume = 66,
      eid = {94},
    pages = {94},
      doi = {10.1093/pasj/psu069},
   adsurl = {http://adsabs.harvard.edu/abs/2014PASJ...66...94B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lodders,
   author = {{Lodders}, K. and {Palme}, H.},
    title = "{Solar System Elemental Abundances in 2009}",
  journal = {Meteoritics and Planetary Science Supplement},
     year = 2009,
    month = sep,
   volume = 72,
    pages = {5154},
   adsurl = {http://adsabs.harvard.edu/abs/2009M%26PSA..72.5154L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{C&M,
   author = {{Chaplin}, W.~J. and {Miglio}, A.},
    title = "{Asteroseismology of Solar-Type and Red-Giant Stars}",
  journal = {ARAA},
archivePrefix = "arXiv",
   eprint = {1303.1957},
 primaryClass = "astro-ph.SR",
     year = 2013,
    month = aug,
   volume = 51,
    pages = {353-392},
      doi = {10.1146/annurev-astro-082812-140938},
   adsurl = {http://adsabs.harvard.edu/abs/2013ARA%26A..51..353C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jimenez,
   author = {{Jimenez}, R. and {Flynn}, C. and {MacDonald}, J. and {Gibson}, B.~K.
	},
    title = "{The Cosmic Production of Helium}",
  journal = {Science},
   eprint = {astro-ph/0303179},
     year = 2003,
    month = mar,
   volume = 299,
    pages = {1552-1555},
      doi = {10.1126/science.1080866},
   adsurl = {http://adsabs.harvard.edu/abs/2003Sci...299.1552J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Serenelli,
   author = {{Serenelli}, A.~M. and {Basu}, S.},
    title = "{Determining the Initial Helium Abundance of the Sun}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1006.0244},
 primaryClass = "astro-ph.SR",
 keywords = {diffusion, Sun: abundances, Sun: helioseismology, Sun: interior},
     year = 2010,
    month = aug,
   volume = 719,
    pages = {865-872},
      doi = {10.1088/0004-637X/719/1/865},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...719..865S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Balser,
   author = {{Balser}, D.~S.},
    title = "{The Chemical Evolution of Helium}",
  journal = {Astronomical Journal},
   eprint = {astro-ph/0608436},
 keywords = {ISM: H II Regions, ISM: Abundances, Radio Lines: ISM},
     year = 2006,
    month = dec,
   volume = 132,
    pages = {2326-2332},
      doi = {10.1086/508515},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....132.2326B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chiappini,
   author = {{Chiappini}, C. and {Renda}, A. and {Matteucci}, F.},
    title = "{Evolution of deuterium, $^{3}$He and $^{4}$He in the Galaxy}",
  journal = {A \& A},
   eprint = {astro-ph/0209240},
 keywords = {Galaxy: abundances, Galaxy: evolution, Galaxy: formation},
     year = 2002,
    month = dec,
   volume = 395,
    pages = {789-801},
      doi = {10.1051/0004-6361:20021314},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...395..789C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Asplund,
   author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J. and {Scott}, P.
	},
    title = "{The Chemical Composition of the Sun}",
  journal = {Annual Review of Astron and Astrophys},
archivePrefix = "arXiv",
   eprint = {0909.0948},
 primaryClass = "astro-ph.SR",
     year = 2009,
    month = sep,
   volume = 47,
    pages = {481-522},
      doi = {10.1146/annurev.astro.46.060407.145222},
   adsurl = {http://adsabs.harvard.edu/abs/2009ARA%26A..47..481A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chiosi,
   author = {{Chiosi}, C. and {Matteucci}, F.~M.},
    title = "{The helium to heavy element enrichment ratio, Delta Y/Delta Z}",
  journal = {A \& A},
 keywords = {Chemical Evolution, Galactic Evolution, Heavy Elements, Helium, Stellar Evolution, Stellar Mass Ejection, Abundance, Astronomical Models, Mass Ratios, Sun},
     year = 1982,
    month = jan,
   volume = 105,
    pages = {140-148},
   adsurl = {http://adsabs.harvard.edu/abs/1982A%26A...105..140C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Casagrande,
   author = {{Casagrande}, L. and {Flynn}, C. and {Portinari}, L. and {Girardi}, L. and 
	{Jimenez}, R.},
    title = "{The helium abundance and {$\Delta$}Y/{$\Delta$}Z in lower main-sequence stars}",
  journal = {MNRAS},
   eprint = {astro-ph/0703766},
 keywords = {stars: abundances, stars: fundamental parameters (colours, luminosities, masses, radii, temperatures, etc.), Hertzsprung-Russell (HR) diagram, binaries: general, stars: interiors, stars: late-type},
     year = 2007,
    month = dec,
   volume = 382,
    pages = {1516-1540},
      doi = {10.1111/j.1365-2966.2007.12512.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382.1516C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Stello,
  author={Dennis Stello and Sarbani Basu and Hans Bruntt and Benoît Mosser and Ian R. Stevens and Timothy M. Brown and Jørgen
Christensen-Dalsgaard and Ronald L. Gilliland and Hans Kjeldsen and Torben Arentoft and Jérôme Ballot and Caroline
Barban and Timothy R. Bedding and William J. Chaplin and Yvonne P. Elsworth and Rafael A. García and Marie-Jo
Goupil and Saskia Hekker and Daniel Huber and Savita Mathur and Søren Meibom and Vinothini Sangaralingam and Charles S.
Baldner and Kevin Belkacem and Katia Biazzo and Karsten Brogaard and Juan Carlos Suárez and Francesca D'Antona and Pierre
Demarque and Lisa Esch and Ning Gai and Frank Grundahl and Yveline Lebreton and Biwei Jiang and Nada Jevtic and Christoffer
Karoff and Andrea Miglio and Joanna Molenda-Żakowicz and Josefina Montalbán and Arlette Noels and Teodoro Roca
Cortés and Ian W. Roxburgh and Aldo M. Serenelli and Victor Silva Aguirre and Christiaan Sterken and Peter Stine and Robert
Szabó and Achim Weiss and William J. Borucki and David Koch and Jon M. Jenkins},
  title={Detection of Solar-like Oscillations from Kepler Photometry of the Open Cluster NGC 6819},
  journal={ApJL},
  volume={713},
  number={2},
  pages={L182},
  url={http://stacks.iop.org/2041-8205/713/i=2/a=L182},
  year={2010},
  abstract={Asteroseismology of stars in clusters has been a long-sought goal because the assumption of a common age, distance, and initial chemical composition allows strong tests of the theory of stellar evolution. We report results from the first 34days of science data from the Kepler Mission for the open cluster NGC 6819—one of the four clusters in the field of view. We obtain the first clear detections of solar-like oscillations in the cluster red giants and are able to measure the large frequency separation, Δν, and the frequency of maximum oscillation power, ν max . We find that the asteroseismic parameters allow us to test cluster membership of the stars, and even with the limited seismic data in hand, we can already identify four possible non-members despite their having a better than 80% membership probability from radial velocity measurements. We are also able to determine the oscillation amplitudes for stars that span about 2 orders of magnitude in luminosity and find good agreement with the prediction that oscillation amplitudes scale as the luminosity to the power of 0.7. These early results demonstrate the unique potential of asteroseismology of the stellar clusters observed by Kepler .}
}
	

@ARTICLE{Marcy,
   author = {{Marcy}, G.~W. and {Isaacson}, H. and {Howard}, A.~W. and {Rowe}, J.~F. and 
	{Jenkins}, J.~M. and {Bryson}, S.~T. and {Latham}, D.~W. and 
	{Howell}, S.~B. and {Gautier}, III, T.~N. and {Batalha}, N.~M. and 
	{Rogers}, L. and {Ciardi}, D. and {Fischer}, D.~A. and {Gilliland}, R.~L. and 
	{Kjeldsen}, H. and {Christensen-Dalsgaard}, J. and {Huber}, D. and 
	{Chaplin}, W.~J. and {Basu}, S. and {Buchhave}, L.~A. and {Quinn}, S.~N. and 
	{Borucki}, W.~J. and {Koch}, D.~G. and {Hunter}, R. and {Caldwell}, D.~A. and 
	{Van Cleve}, J. and {Kolbl}, R. and {Weiss}, L.~M. and {Petigura}, E. and 
	{Seager}, S. and {Morton}, T. and {Johnson}, J.~A. and {Ballard}, S. and 
	{Burke}, C. and {Cochran}, W.~D. and {Endl}, M. and {MacQueen}, P. and 
	{Everett}, M.~E. and {Lissauer}, J.~J. and {Ford}, E.~B. and 
	{Torres}, G. and {Fressin}, F. and {Brown}, T.~M. and {Steffen}, J.~H. and 
	{Charbonneau}, D. and {Basri}, G.~S. and {Sasselov}, D.~D. and 
	{Winn}, J. and {Sanchis-Ojeda}, R. and {Christiansen}, J. and 
	{Adams}, E. and {Henze}, C. and {Dupree}, A. and {Fabrycky}, D.~C. and 
	{Fortney}, J.~J. and {Tarter}, J. and {Holman}, M.~J. and {Tenenbaum}, P. and 
	{Shporer}, A. and {Lucas}, P.~W. and {Welsh}, W.~F. and {Orosz}, J.~A. and 
	{Bedding}, T.~R. and {Campante}, T.~L. and {Davies}, G.~R. and 
	{Elsworth}, Y. and {Handberg}, R. and {Hekker}, S. and {Karoff}, C. and 
	{Kawaler}, S.~D. and {Lund}, M.~N. and {Lundkvist}, M. and {Metcalfe}, T.~S. and 
	{Miglio}, A. and {Silva Aguirre}, V. and {Stello}, D. and {White}, T.~R. and 
	{Boss}, A. and {Devore}, E. and {Gould}, A. and {Prsa}, A. and 
	{Agol}, E. and {Barclay}, T. and {Coughlin}, J. and {Brugamyer}, E. and 
	{Mullally}, F. and {Quintana}, E.~V. and {Still}, M. and {Thompson}, S.~E. and 
	{Morrison}, D. and {Twicken}, J.~D. and {D{\'e}sert}, J.-M. and 
	{Carter}, J. and {Crepp}, J.~R. and {H{\'e}brard}, G. and {Santerne}, A. and 
	{Moutou}, C. and {Sobeck}, C. and {Hudgins}, D. and {Haas}, M.~R. and 
	{Robertson}, P. and {Lillo-Box}, J. and {Barrado}, D.},
    title = "{Masses, Radii, and Orbits of Small Kepler Planets: The Transition from Gaseous to Rocky Planets}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1401.4195},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems, planets and satellites: detection, stars: individual: Kepler-25 Kepler-37 Kepler-48 Kepler-68 Kepler-93 Kepler-94 Kepler-95 Kepler-96 Kepler-97 Kepler-98 Kepler-99 Kepler-100 Kepler-102 Kepler-103 Kepler-106 Kepler-109 Kepler-113 Kepler-131 Kepler-406 Kepler-407 Kepler-409, techniques: photometric, techniques: radial velocities},
     year = 2014,
    month = feb,
   volume = 210,
      eid = {20},
    pages = {20},
      doi = {10.1088/0067-0049/210/2/20},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..210...20M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{nsamba,
   author = {{Nsamba}, B. and {Monteiro}, M.~J.~P.~F.~G. and {Campante}, T.~L. and 
	{Reese}, D.~R. and {White}, T.~R. and {Garc{\'{\i}}a Hern{\'a}ndez}, A. and 
	{Jiang}, C.},
    title = "{Asteroseismic modelling of the Binary HD 176465}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1611.05698},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics},
     year = 2016,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161105698N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{white,
   author = {{White}, T.~R. and {Benomar}, O. and {Silva Aguirre}, V. and 
	{Ball}, W.~H. and {Bedding}, T.~R. and {Chaplin}, W.~J. and 
	{Christensen-Dalsgaard}, J. and {Garcia}, R.~A. and {Gizon}, L. and 
	{Stello}, D. and {Aigrain}, S. and {Antia}, H.~M. and {Appourchaux}, T. and 
	{Bazot}, M. and {Campante}, T.~L. and {Creevey}, O.~L. and {Davies}, G.~R. and 
	{Elsworth}, Y.~P. and {Gaulme}, P. and {Handberg}, R. and {Hekker}, S. and 
	{Houdek}, G. and {Howe}, R. and {Huber}, D. and {Karoff}, C. and 
	{Marques}, J.~P. and {Mathur}, S. and {McQuillan}, A. and {Metcalfe}, T.~S. and 
	{Mosser}, B. and {Nielsen}, M.~B. and {R{\'e}gulo}, C. and {Salabert}, D. and 
	{Stahn}, T.},
    title = "{Kepler observations of the asteroseismic binary HD 176465}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1609.09581},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, methods: data analysis, stars: individual: HD 176465},
     year = 2017,
    month = may,
   volume = 601,
      eid = {A82},
    pages = {A82},
      doi = {10.1051/0004-6361/201628706},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...601A..82W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Metcalfe,
   author = {{Metcalfe}, T.~S. and {Creevey}, O.~L. and {Do{\u g}an}, G. and 
	{Mathur}, S. and {Xu}, H. and {Bedding}, T.~R. and {Chaplin}, W.~J. and 
	{Christensen-Dalsgaard}, J. and {Karoff}, C. and {Trampedach}, R. and 
	{Benomar}, O. and {Brown}, B.~P. and {Buzasi}, D.~L. and {Campante}, T.~L. and 
	{{\c C}elik}, Z. and {Cunha}, M.~S. and {Davies}, G.~R. and 
	{Deheuvels}, S. and {Derekas}, A. and {Di Mauro}, M.~P. and 
	{Garc{\'{\i}}a}, R.~A. and {Guzik}, J.~A. and {Howe}, R. and 
	{MacGregor}, K.~B. and {Mazumdar}, A. and {Montalb{\'a}n}, J. and 
	{Monteiro}, M.~J.~P.~F.~G. and {Salabert}, D. and {Serenelli}, A. and 
	{Stello}, D. and {Ste{\amp}{\c s}acute} and {licki}, M. and 
	{Suran}, M.~D. and {Y{\i}ld{\i}z}, M. and {Aksoy}, C. and {Elsworth}, Y. and 
	{Gruberbauer}, M. and {Guenther}, D.~B. and {Lebreton}, Y. and 
	{Molaverdikhani}, K. and {Pricopi}, D. and {Simoniello}, R. and 
	{White}, T.~R.},
    title = "{Properties of 42 Solar-type Kepler Targets from the Asteroseismic Modeling Portal}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1402.3614},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, stars: evolution, stars: interiors, stars: oscillations},
     year = 2014,
    month = oct,
   volume = 214,
      eid = {27},
    pages = {27},
      doi = {10.1088/0067-0049/214/2/27},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..214...27M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Guzik,
   author = {{Guzik}, J.~A. and {Cox}, A.~N.},
    title = "{Using solar p-modes to determine the convection zone depth and constrain diffusion-produced composition gradients}",
  journal = {ApJ},
 keywords = {Convection, Equations Of State, Gaseous Diffusion, Helium Atoms, Solar Interior, Solar Oscillations, Abundance, Gas Ionization, Turbulent Mixing, Weighting Functions},
     year = 1993,
    month = jul,
   volume = 411,
    pages = {394-401},
      doi = {10.1086/172840},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...411..394G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Aller,
   author = {{Aller}, L.~H. and {Chapman}, S.},
    title = "{Diffusion in the Sun.}",
  journal = {ApJ},
     year = 1960,
    month = sep,
   volume = 132,
    pages = {461},
      doi = {10.1086/146943},
   adsurl = {http://adsabs.harvard.edu/abs/1960ApJ...132..461A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Korn,
   author = {{Korn}, A.~J. and {Grundahl}, F. and {Richard}, O. and {Mashonkina}, L. and 
	{Barklem}, P.~S. and {Collet}, R. and {Gustafsson}, B. and {Piskunov}, N.
	},
    title = "{Atomic Diffusion and Mixing in Old Stars. I. Very Large Telescope FLAMES-UVES Observations of Stars in NGC 6397}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {0709.0639},
 keywords = {Diffusion, Galaxy: Globular Clusters: Individual: NGC Number: NGC 6397, Stars: Abundances, Stars: Atmospheres, Stars: Evolution, Stars: Fundamental Parameters, Stars: Interiors, Stars: Population II},
     year = 2007,
    month = dec,
   volume = 671,
    pages = {402-419},
      doi = {10.1086/523098},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...671..402K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dalsgaard,
   author = {{Christensen-Dalsgaard}, J. and {Thompson}, M.~J.},
    title = "{On solar p-mode frequency shifts caused by near-surface model changes}",
  journal = {MNRAS},
 keywords = {SUN, INTERIOR - SUN, OSCILLATIONS},
     year = 1997,
    month = jan,
   volume = 284,
    pages = {527-540},
      doi = {10.1093/mnras/284.3.527},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.284..527C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brand,
   author = {{Brand{\~a}o}, I.~M. and {Do{\u g}an}, G. and {Christensen-Dalsgaard}, J. and 
	{Cunha}, M.~S. and {Bedding}, T.~R. and {Metcalfe}, T.~S. and 
	{Kjeldsen}, H. and {Bruntt}, H. and {Arentoft}, T.},
    title = "{Asteroseismic modelling of the solar-type subgiant star {$\beta$} Hydri}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1012.3872},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: solar-type, stars:, individual:{$\beta$}Hydri},
     year = 2011,
    month = mar,
   volume = 527,
      eid = {A37},
    pages = {A37},
      doi = {10.1051/0004-6361/201015370},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...527A..37B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chap,
   author = {{Chaplin}, W.~J. and {Basu}, S. and {Huber}, D. and {Serenelli}, A. and 
	{Casagrande}, L. and {Silva Aguirre}, V. and {Ball}, W.~H. and 
	{Creevey}, O.~L. and {Gizon}, L. and {Handberg}, R. and {Karoff}, C. and 
	{Lutz}, R. and {Marques}, J.~P. and {Miglio}, A. and {Stello}, D. and 
	{Suran}, M.~D. and {Pricopi}, D. and {Metcalfe}, T.~S. and {Monteiro}, M.~J.~P.~F.~G. and 
	{Molenda-{\.Z}akowicz}, J. and {Appourchaux}, T. and {Christensen-Dalsgaard}, J. and 
	{Elsworth}, Y. and {Garc{\'{\i}}a}, R.~A. and {Houdek}, G. and 
	{Kjeldsen}, H. and {Bonanno}, A. and {Campante}, T.~L. and {Corsaro}, E. and 
	{Gaulme}, P. and {Hekker}, S. and {Mathur}, S. and {Mosser}, B. and 
	{R{\'e}gulo}, C. and {Salabert}, D.},
    title = "{Asteroseismic Fundamental Properties of Solar-type Stars Observed by the NASA Kepler Mission}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1310.4001},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, methods: data analysis, stars: fundamental parameters, stars: interiors },
     year = 2014,
    month = jan,
   volume = 210,
      eid = {1},
    pages = {1},
      doi = {10.1088/0067-0049/210/1/1},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..210....1C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Campante,
   author = {{Campante}, T.~L. and {Schofield}, M. and {Kuszlewicz}, J.~S. and 
	{Bouma}, L. and {Chaplin}, W.~J. and {Huber}, D. and {Christensen-Dalsgaard}, J. and 
	{Kjeldsen}, H. and {Bossini}, D. and {North}, T.~S.~H. and {Appourchaux}, T. and 
	{Latham}, D.~W. and {Pepper}, J. and {Ricker}, G.~R. and {Stassun}, K.~G. and 
	{Vanderspek}, R. and {Winn}, J.~N.},
    title = "{The Asteroseismic Potential of TESS: Exoplanet-host Stars}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1608.01138},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, planets and satellites: detection, space vehicles: instruments, surveys, techniques: photometric },
     year = 2016,
    month = oct,
   volume = 830,
      eid = {138},
    pages = {138},
      doi = {10.3847/0004-637X/830/2/138},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...830..138C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Rauer,
   author = {{Rauer}, H. and {Aerts}, C. and {Cabrera}, J. and {PLATO Team}
	},
    title = "{The PLATO Mission}",
  journal = {Astronomische Nachrichten},
 keywords = {Stellar ages, asteroseismology, planetary systems, space vehicles, space vehicles: instruments, stars: evolution, techniques: photometric},
     year = 2016,
    month = sep,
   volume = 337,
    pages = {961},
      doi = {10.1002/asna.201612408},
   adsurl = {http://adsabs.harvard.edu/abs/2016AN....337..961R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Rox,
   author = {{Roxburgh}, I.~W. and {Vorontsov}, S.~V.},
  journal = {A \& A},
 keywords = {stars: oscillations},
     year = 2003,
    month = nov,
   volume = 411,
    pages = {215-220},
      doi = {10.1051/0004-6361:20031318},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411..215R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Broomhall,
   author = {{Broomhall}, A.-M. and {Chaplin}, W.~J. and {Davies}, G.~R. and 
	{Elsworth}, Y. and {Fletcher}, S.~T. and {Hale}, S.~J. and {Miller}, B. and 
	{New}, R.},
    title = "{Definitive Sun-as-a-star p-mode frequencies: 23 years of BiSON observations}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {0903.5219},
 primaryClass = "astro-ph.SR",
 keywords = {methods: data analysis, Sun: oscillations},
     year = 2009,
    month = jun,
   volume = 396,
    pages = {L100-L104},
      doi = {10.1111/j.1745-3933.2009.00672.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396L.100B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Borucki,
   author = {{Borucki}, W.~J. and {Koch}, D. and {Basri}, G. and {Batalha}, N. and 
	{Brown}, T. and {Caldwell}, D. and {Caldwell}, J. and {Christensen-Dalsgaard}, J. and 
	{Cochran}, W.~D. and {DeVore}, E. and {Dunham}, E.~W. and {Dupree}, A.~K. and 
	{Gautier}, T.~N. and {Geary}, J.~C. and {Gilliland}, R. and 
	{Gould}, A. and {Howell}, S.~B. and {Jenkins}, J.~M. and {Kondo}, Y. and 
	{Latham}, D.~W. and {Marcy}, G.~W. and {Meibom}, S. and {Kjeldsen}, H. and 
	{Lissauer}, J.~J. and {Monet}, D.~G. and {Morrison}, D. and 
	{Sasselov}, D. and {Tarter}, J. and {Boss}, A. and {Brownlee}, D. and 
	{Owen}, T. and {Buzasi}, D. and {Charbonneau}, D. and {Doyle}, L. and 
	{Fortney}, J. and {Ford}, E.~B. and {Holman}, M.~J. and {Seager}, S. and 
	{Steffen}, J.~H. and {Welsh}, W.~F. and {Rowe}, J. and {Anderson}, H. and 
	{Buchhave}, L. and {Ciardi}, D. and {Walkowicz}, L. and {Sherry}, W. and 
	{Horch}, E. and {Isaacson}, H. and {Everett}, M.~E. and {Fischer}, D. and 
	{Torres}, G. and {Johnson}, J.~A. and {Endl}, M. and {MacQueen}, P. and 
	{Bryson}, S.~T. and {Dotson}, J. and {Haas}, M. and {Kolodziejczak}, J. and 
	{Van Cleve}, J. and {Chandrasekaran}, H. and {Twicken}, J.~D. and 
	{Quintana}, E.~V. and {Clarke}, B.~D. and {Allen}, C. and {Li}, J. and 
	{Wu}, H. and {Tenenbaum}, P. and {Verner}, E. and {Bruhweiler}, F. and 
	{Barnes}, J. and {Prsa}, A.},
    title = "{Kepler Planet-Detection Mission: Introduction and First Results}",
  journal = {Science},
     year = 2010,
    month = feb,
   volume = 327,
    pages = {977},
      doi = {10.1126/science.1185402},
   adsurl = {http://adsabs.harvard.edu/abs/2010Sci...327..977B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gruberbauer,
   author = {{Gruberbauer}, M. and {Guenther}, D.~B. and {MacLeod}, K. and 
	{Kallinger}, T.},
    title = "{Bayesian asteroseismology of 23 solar-like Kepler targets}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1307.4218},
 primaryClass = "astro-ph.SR",
 keywords = {methods: statistical, stars: oscillations},
     year = 2013,
    month = oct,
   volume = 435,
    pages = {242-254},
      doi = {10.1093/mnras/stt1289},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435..242G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BedKj,
   author = {{Bedding}, T.~R. and {Kjeldsen}, H.},
    title = "{Solar-like Oscillations}",
  journal = {PASA},
   eprint = {astro-ph/0305425},
 keywords = {stars: oscillations},
     year = 2003,
   volume = 20,
    pages = {203-212},
      doi = {10.1071/AS03025},
   adsurl = {http://adsabs.harvard.edu/abs/2003PASA...20..203B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vauclair,
   author = {{Th{\'e}ado}, S. and {Vauclair}, S. and {Castro}, M. and {Charpinet}, S. and 
	{Dolez}, N.},
    title = "{Asteroseismic tests of element diffusion in solar type stars}",
  journal = {A&A},
 keywords = {diffusion, hydrodynamics, stars: abundances, stars: interiors, stars: oscillations (including pulsations)},
     year = 2005,
    month = jul,
   volume = 437,
    pages = {553-560},
      doi = {10.1051/0004-6361:20042328},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...437..553T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Deal,
   author = {{Deal}, M. and {Escobar}, M.~E. and {Vauclair}, S. and {Vauclair}, G. and 
	{Hui-Bon-Hoa}, A. and {Richard}, O.},
    title = "{Asteroseismology of the exoplanet-host F-type star 94 Ceti: Impact of atomic diffusion on the stellar parameters}",
  journal = {A&A},
archivePrefix = "arXiv",
   eprint = {1702.03170},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, planetary systems, diffusion, instabilities, stars: evolution},
     year = 2017,
    month = may,
   volume = 601,
      eid = {A127},
    pages = {A127},
      doi = {10.1051/0004-6361/201629825},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...601A.127D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Verma,
   author = {{Verma}, K. and {Hanasoge}, S. and {Bhattacharya}, J. and {Antia}, H.~M. and 
	{Krishnamurthi}, G.},
    title = "{Asteroseismic determination of fundamental parameters of Sun-like stars using multilayered neural networks}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1602.00902},
 primaryClass = "astro-ph.SR",
 keywords = {stars: fundamental parameters, stars: interiors, stars: low-mass, stars: oscillations, stars: solar-type},
     year = 2016,
    month = oct,
   volume = 461,
    pages = {4206-4214},
      doi = {10.1093/mnras/stw1621},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.461.4206V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Perryman,
   author = {{Perryman}, M.~A.~C. and {de Boer}, K.~S. and {Gilmore}, G. and 
	{H{\o}g}, E. and {Lattanzi}, M.~G. and {Lindegren}, L. and {Luri}, X. and 
	{Mignard}, F. and {Pace}, O. and {de Zeeuw}, P.~T.},
    title = "{GAIA: Composition, formation and evolution of the Galaxy}",
  journal = {A&A},
   eprint = {astro-ph/0101235},
 keywords = {INSTRUMENTATION: MISCELLANEOUS, SPACE VEHICLES: INSTRUMENTS, ASTROMETRY, GALAXY: GENERAL, TECHNIQUES: PHOTOMETRIC, TECHNIQUES: RADIAL VELOCITIES},
     year = 2001,
    month = apr,
   volume = 369,
    pages = {339-363},
      doi = {10.1051/0004-6361:20010085},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...369..339P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{mos,
	author = {{Mosser}, B. and {Michel, E.} and {Belkacem, K.} and {Goupil, M. J.} and {Baglin, A.} and {Barban, C.} and {Provost, J.} and {Samadi, R.} and {Auvergne, M.} and {Catala, C.}},
	title = {Asymptotic and measured large frequency separations⋆},
	DOI= "10.1051/0004-6361/201220435",
	url= "https://doi.org/10.1051/0004-6361/201220435",
	journal = {A&A},
	year = 2013,
	volume = 550,
	pages = "A126",
	month = "",
}

@article{Mamajek,
  author={ Eric E. Mamajek },
  title={On the Age and Binarity of Fomalhaut},
  journal={ApJL},
  volume={754},
  number={2},
  pages={L20},
  url={http://stacks.iop.org/2041-8205/754/i=2/a=L20},
  year={2012},
  abstract={The nearby ( d = 7.7pc) A3V star Fomalhaut is orbited by a resolved dusty debris disk and a controversial candidate extrasolar planet. The commonly cited age for the system (200 ± 100Myr) from Barrado y Navascues et al. relied on a combination of isochronal age plus youth indicators for the K4V common proper-motion system TW PsA. TW PsA is 1 ##IMG## [http://ej.iop.org/icons/Entities/fdg.gif] {fdg} 96 away from Fomalhaut and was first proposed as a companion by Luyten, but the physicality of the binarity is worth testing with modern data. I demonstrate that TW PsA is unequivocally a physical stellar companion to Fomalhaut, with true separation 0.280 +0.019 – 0.012pc (57.4 +3.9 – 2.5kAU) and sharing velocities within 0.1±0.5kms –1 —consistent with being a bound system. Hence, TW PsA should be considered "FomalhautB." Combining modern H-R diagram constraints with four sets of evolutionary tracks, and assuming the star was born with protosolar composition, I estimate a new isochronal age for Fomalhaut of 450 ± 40Myr and mass of 1.92±0.02 M ☉ . Various stellar youth diagnostics are re-examined for TW PsA. The star's rotation, X-ray emission, and Li abundances are consistent with approximate ages of 410, 380, and 360Myr, respectively, yielding a weighted mean age of 400 ± 70Myr. Combining the independent ages, I estimate a mean age for the Fomalhaut-TW PsA binary of 440 ± 40Myr. The older age implies that substellar companions of a given mass are approximately 1mag fainter at IR wavelengths than previously assumed.}
}

@ARTICLE{Figueira,
   author = {{Figueira}, P. and {Faria}, J.~P. and {Adibekyan}, V.~Z. and 
	{Oshagh}, M. and {Santos}, N.~C.},
    title = "{A Pragmatic Bayesian Perspective on Correlation Analysis. The exoplanetary gravity - stellar activity case}",
  journal = {Origins of Life and Evolution of the Biosphere},
archivePrefix = "arXiv",
   eprint = {1601.05107},
 primaryClass = "astro-ph.IM",
 keywords = {Exoplanets, Stellar activity, Statistics, Correlations},
     year = 2016,
    month = nov,
   volume = 46,
    pages = {385-393},
      doi = {10.1007/s11084-016-9490-5},
   adsurl = {http://adsabs.harvard.edu/abs/2016OLEB...46..385F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Ben,
	author = {{Nsamba}, B. and {Monteiro}, M. J. P. F. G. and {Campante}, T. L. and {Reese}, D. R. and {White}, T. R. and {Garc\'ia Hern\'andez}, A. and {Jiang}, C.},
	title = {Asteroseismic modelling of the Binary HD 176465},
	DOI= "10.1051/epjconf/201716005010",
	url= "https://doi.org/10.1051/epjconf/201716005010",
	journal = {EPJ Web Conf.},
	year = 2017,
	volume = 160,
	pages = "05010",
}

@ARTICLE{Nordlund,
   author = {{Trampedach}, R. and {Stein}, R.~F. and {Christensen-Dalsgaard}, J. and 
	{Nordlund}, {\AA}. and {Asplund}, M.},
    title = "{Improvements to stellar structure models, based on a grid of 3D convection simulations - II. Calibrating the mixing-length formulation}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1410.1559},
 primaryClass = "astro-ph.SR",
 keywords = {convection, stars: atmospheres, stars: evolution},
     year = 2014,
    month = dec,
   volume = 445,
    pages = {4366-4384},
      doi = {10.1093/mnras/stu2084},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.445.4366T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{CTL,
   author = {{Campante}, T.~L. and {Lund}, M.~N. and {Kuszlewicz}, J.~S. and 
	{Davies}, G.~R. and {Chaplin}, W.~J. and {Albrecht}, S. and 
	{Winn}, J.~N. and {Bedding}, T.~R. and {Benomar}, O. and {Bossini}, D. and 
	{Handberg}, R. and {Santos}, A.~R.~G. and {Van Eylen}, V. and 
	{Basu}, S. and {Christensen-Dalsgaard}, J. and {Elsworth}, Y.~P. and 
	{Hekker}, S. and {Hirano}, T. and {Huber}, D. and {Karoff}, C. and 
	{Kjeldsen}, H. and {Lundkvist}, M.~S. and {North}, T.~S.~H. and 
	{Silva Aguirre}, V. and {Stello}, D. and {White}, T.~R.},
    title = "{Spin-Orbit Alignment of Exoplanet Systems: Ensemble Analysis Using Asteroseismology}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1601.06052},
 primaryClass = "astro-ph.EP",
 keywords = {asteroseismology, methods: statistical, planetary systems, planets and satellites: general, stars: solar-type, techniques: photometric},
     year = 2016,
    month = mar,
   volume = 819,
      eid = {85},
    pages = {85},
      doi = {10.3847/0004-637X/819/1/85},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...819...85C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}

@ARTICLE{Kawa,
   author = {{Chaplin}, W.~J. and {Sanchis-Ojeda}, R. and {Campante}, T.~L. and 
	{Handberg}, R. and {Stello}, D. and {Winn}, J.~N. and {Basu}, S. and 
	{Christensen-Dalsgaard}, J. and {Davies}, G.~R. and {Metcalfe}, T.~S. and 
	{Buchhave}, L.~A. and {Fischer}, D.~A. and {Bedding}, T.~R. and 
	{Cochran}, W.~D. and {Elsworth}, Y. and {Gilliland}, R.~L. and 
	{Hekker}, S. and {Huber}, D. and {Isaacson}, H. and {Karoff}, C. and 
	{Kawaler}, S.~D. and {Kjeldsen}, H. and {Latham}, D.~W. and 
	{Lund}, M.~N. and {Lundkvist}, M. and {Marcy}, G.~W. and {Miglio}, A. and 
	{Barclay}, T. and {Lissauer}, J.~J.},
    title = "{Asteroseismic Determination of Obliquities of the Exoplanet Systems Kepler-50 and Kepler-65}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1302.3728},
 primaryClass = "astro-ph.EP",
 keywords = {asteroseismology, planets and satellites: formation, planets and satellites: general, stars: rotation },
     year = 2013,
    month = apr,
   volume = 766,
      eid = {101},
    pages = {101},
      doi = {10.1088/0004-637X/766/2/101},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...766..101C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{SCM,
   author = {{Campante}, T.~L. and {Santos}, N.~C. and {Monteiro}, M.~J.~P.~F.~G.
	},
    title = "{Asteroseismology and Exoplanets: Proceedings of the IVth Azores International Advanced School in Space Sciences}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1709.00645},
 primaryClass = "astro-ph.SR",
 keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
     year = 2017,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170900645C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Schwarzschild,
   author = {{Schwarzschild}, M.},
    title = "{Structure and evolution of the stars.}",
 keywords = {STARS: STRUCTURE, STARS: EVOLUTION},
booktitle = {Princeton, Princeton University Press, 1958.},
     year = 1958,
   adsurl = {http://adsabs.harvard.edu/abs/1958ses..book.....S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{WHG,
   author = {{Ball}, W.~H. and {Gizon}, L.},
    title = "{Surface-effect corrections for oscillation frequencies of evolved stars}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1702.02570},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: oscillations},
     year = 2017,
    month = apr,
   volume = 600,
      eid = {A128},
    pages = {A128},
      doi = {10.1051/0004-6361/201630260},
   adsurl = {http://adsabs.harvard.edu/abs/2017A%26A...600A.128B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@BOOK{Allen,
   author = {{Allen}, C.~W.},
    title = "{Astrophysical Quantities}",
booktitle = {Astrophysical Quantities, London: Athlone (3rd edition), 1976},
     year = 1976,
   adsurl = {http://adsabs.harvard.edu/abs/1976asqu.book.....A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kjeldsen2,
   author = {{Kjeldsen}, H. and {Bedding}, T.~R.},
    title = "{Amplitudes of stellar oscillations: the implications for asteroseismology.}",
  journal = {\aap},
   eprint = {astro-ph/9403015},
 keywords = {SUN: OSCILLATIONS, STARS: INDIVIDUAL: $\{$ALPHA$\}$ CEN, STARS: INDIVIDUAL: PROCYON, STARS: OSCILLATIONS, CEPHEIDS, $\{$DELTA$\}$ SCT},
     year = 1995,
    month = jan,
   volume = 293,
    pages = {87-106},
   adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...293...87K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Brown,
   author = {{Brown}, T.~M. and {Gilliland}, R.~L. and {Noyes}, R.~W. and 
	{Ramsey}, L.~W.},
    title = "{Detection of possible p-mode oscillations on Procyon}",
  journal = {ApJ},
 keywords = {F Stars, Late Stars, Stellar Oscillations, Subgiant Stars, Charge Coupled Devices, Doppler Effect, Power Spectra, Stellar Luminosity, Stellar Temperature},
     year = 1991,
    month = feb,
   volume = 368,
    pages = {599-609},
      doi = {10.1086/169725},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...368..599B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Eylen,
   author = {{Van Eylen}, V. and {Kjeldsen}, H. and {Christensen-Dalsgaard}, J. and 
	{Aerts}, C.},
    title = "{Properties of extrasolar planets and their host stars: A case study of HAT-P-7}",
  journal = {Astronomische Nachrichten},
archivePrefix = "arXiv",
   eprint = {1301.1472},
 primaryClass = "astro-ph.SR",
 keywords = {planetary systems, stars: fundamental parameters, stars: individual (HAT-P-7), stars: oscillations},
     year = 2012,
    month = dec,
   volume = 333,
    pages = {1088},
      doi = {10.1002/asna.201211832},
   adsurl = {http://adsabs.harvard.edu/abs/2012AN....333.1088V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Huber,
   author = {{Huber}, D. and {Chaplin}, W.~J. and {Christensen-Dalsgaard}, J. and 
	{Gilliland}, R.~L. and {Kjeldsen}, H. and {Buchhave}, L.~A. and 
	{Fischer}, D.~A. and {Lissauer}, J.~J. and {Rowe}, J.~F. and 
	{Sanchis-Ojeda}, R. and {Basu}, S. and {Handberg}, R. and {Hekker}, S. and 
	{Howard}, A.~W. and {Isaacson}, H. and {Karoff}, C. and {Latham}, D.~W. and 
	{Lund}, M.~N. and {Lundkvist}, M. and {Marcy}, G.~W. and {Miglio}, A. and 
	{Silva Aguirre}, V. and {Stello}, D. and {Arentoft}, T. and 
	{Barclay}, T. and {Bedding}, T.~R. and {Burke}, C.~J. and {Christiansen}, J.~L. and 
	{Elsworth}, Y.~P. and {Haas}, M.~R. and {Kawaler}, S.~D. and 
	{Metcalfe}, T.~S. and {Mullally}, F. and {Thompson}, S.~E.},
    title = "{Fundamental Properties of Kepler Planet-candidate Host Stars using Asteroseismology}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1302.2624},
 primaryClass = "astro-ph.SR",
 keywords = {planetary systems, stars: late-type, stars: oscillations, techniques: photometric, techniques: spectroscopic},
     year = 2013,
    month = apr,
   volume = 767,
      eid = {127},
    pages = {127},
      doi = {10.1088/0004-637X/767/2/127},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...767..127H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Camp,
   author = {{Campante}, T.~L. and {Barclay}, T. and {Swift}, J.~J. and {Huber}, D. and 
	{Adibekyan}, V.~Z. and {Cochran}, W. and {Burke}, C.~J. and 
	{Isaacson}, H. and {Quintana}, E.~V. and {Davies}, G.~R. and 
	{Silva Aguirre}, V. and {Ragozzine}, D. and {Riddle}, R. and 
	{Baranec}, C. and {Basu}, S. and {Chaplin}, W.~J. and {Christensen-Dalsgaard}, J. and 
	{Metcalfe}, T.~S. and {Bedding}, T.~R. and {Handberg}, R. and 
	{Stello}, D. and {Brewer}, J.~M. and {Hekker}, S. and {Karoff}, C. and 
	{Kolbl}, R. and {Law}, N.~M. and {Lundkvist}, M. and {Miglio}, A. and 
	{Rowe}, J.~F. and {Santos}, N.~C. and {Van Laerhoven}, C. and 
	{Arentoft}, T. and {Elsworth}, Y.~P. and {Fischer}, D.~A. and 
	{Kawaler}, S.~D. and {Kjeldsen}, H. and {Lund}, M.~N. and {Marcy}, G.~W. and 
	{Sousa}, S.~G. and {Sozzetti}, A. and {White}, T.~R.},
    title = "{An Ancient Extrasolar System with Five Sub-Earth-size Planets}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1501.06227},
 primaryClass = "astro-ph.EP",
 keywords = {Galaxy: disk, planetary systems, stars: individual: HIP 94931, stars: late-type, stars: oscillations, techniques: photometric },
     year = 2015,
    month = feb,
   volume = 799,
      eid = {170},
    pages = {170},
      doi = {10.1088/0004-637X/799/2/170},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...799..170C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Thompson,
   author = {{Metcalfe}, T.~S. and {Monteiro}, M.~J.~P.~F.~G. and {Thompson}, M.~J. and 
	{Molenda-{\.Z}akowicz}, J. and {Appourchaux}, T. and {Chaplin}, W.~J. and 
	{Do{\v g}an}, G. and {Eggenberger}, P. and {Bedding}, T.~R. and 
	{Bruntt}, H. and {Creevey}, O.~L. and {Quirion}, P.-O. and {Stello}, D. and 
	{Bonanno}, A. and {Silva Aguirre}, V. and {Basu}, S. and {Esch}, L. and 
	{Gai}, N. and {Di Mauro}, M.~P. and {Kosovichev}, A.~G. and 
	{Kitiashvili}, I.~N. and {Su{\'a}rez}, J.~C. and {Moya}, A. and 
	{Piau}, L. and {Garc{\'{\i}}a}, R.~A. and {Marques}, J.~P. and 
	{Frasca}, A. and {Biazzo}, K. and {Sousa}, S.~G. and {Dreizler}, S. and 
	{Bazot}, M. and {Karoff}, C. and {Frandsen}, S. and {Wilson}, P.~A. and 
	{Brown}, T.~M. and {Christensen-Dalsgaard}, J. and {Gilliland}, R.~L. and 
	{Kjeldsen}, H. and {Campante}, T.~L. and {Fletcher}, S.~T. and 
	{Handberg}, R. and {R{\'e}gulo}, C. and {Salabert}, D. and {Schou}, J. and 
	{Verner}, G.~A. and {Ballot}, J. and {Broomhall}, A.-M. and 
	{Elsworth}, Y. and {Hekker}, S. and {Huber}, D. and {Mathur}, S. and 
	{New}, R. and {Roxburgh}, I.~W. and {Sato}, K.~H. and {White}, T.~R. and 
	{Borucki}, W.~J. and {Koch}, D.~G. and {Jenkins}, J.~M.},
    title = "{A Precise Asteroseismic Age and Radius for the Evolved Sun-like Star KIC 11026764}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1010.4329},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: individual: KIC 11026764, stars: interiors, stars: oscillations},
     year = 2010,
    month = nov,
   volume = 723,
    pages = {1583-1598},
      doi = {10.1088/0004-637X/723/2/1583},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...723.1583M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kjeld,
   author = {{Kjeldsen}, H. and {Bedding}, T.~R. and {Christensen-Dalsgaard}, J.
	},
    title = "{Correcting Stellar Oscillation Frequencies for Near-Surface Effects}",
  journal = {ApJL},
archivePrefix = "arXiv",
   eprint = {0807.1769},
 keywords = {stars: individual: {$\beta$} Hyi {$\alpha$} Cen A {$\alpha$} Cen B, stars: oscillations, Sun: helioseismology},
     year = 2008,
    month = aug,
   volume = 683,
      eid = {L175},
    pages = {L175},
      doi = {10.1086/591667},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...683L.175K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dalsgaard1,
   author = {{Christensen-Dalsgaard}, J. and {Dappen}, W. and {Lebreton}, Y.
	},
    title = "{Solar oscillation frequencies and the equation of state}",
  journal = {Nature},
 keywords = {Equations Of State, Helioseismology, Magnetohydrodynamics, Solar Oscillations, Convection Currents, Stellar Evolution, Stellar Models, Stellar Structure},
     year = 1988,
    month = dec,
   volume = 336,
    pages = {634-638},
      doi = {10.1038/336634a0},
   adsurl = {http://adsabs.harvard.edu/abs/1988Natur.336..634C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dziembowski,
   author = {{Dziembowski}, W.~A. and {Paterno}, L. and {Ventura}, R.},
    title = "{How comparison between observed and calculated p-mode eigenfrequencies can give information on the internal structure of the sun}",
  journal = {A \& A},
 keywords = {Solar Oscillations, Stellar Structure, Vibration Mode, Frequency Distribution, Stellar Models},
     year = 1988,
    month = jul,
   volume = 200,
    pages = {213-217},
   adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...200..213D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chaboyer,
   author = {{Chaboyer}, B. and {Fenton}, W.~H. and {Nelan}, J.~E. and {Patnaude}, D.~J. and 
	{Simon}, F.~E.},
    title = "{Heavy-Element Diffusion in Metal-poor Stars}",
  journal = {ApJ},
   eprint = {astro-ph/0108119},
 keywords = {Diffusion, Galaxy: Globular Clusters: Individual: NGC Number: NGC 6397, Stars: Abundances, Stars: Evolution, Stars: Subdwarfs},
     year = 2001,
    month = nov,
   volume = 562,
    pages = {521-527},
      doi = {10.1086/323872},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...562..521C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dotter,
   author = {{Dotter}, A. and {Conroy}, C. and {Cargile}, P. and {Asplund}, M.
	},
    title = "{The Influence of Atomic Diffusion on Stellar Ages and Chemical Tagging}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1704.03465},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: evolution },
     year = 2017,
    month = may,
   volume = 840,
      eid = {99},
    pages = {99},
      doi = {10.3847/1538-4357/aa6d10},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...840...99D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Christensen,
   author = {{Christensen-Dalsgaard}, J. and {Proffitt}, C.~R. and {Thompson}, M.~J.
	},
    title = "{Effects of diffusion on solar models and their oscillation frequencies}",
  journal = {ApJ},
 keywords = {Plasma Diffusion, Solar Interior, Solar Oscillations, Asymptotic Properties, Frequencies, Helium, Stellar Models},
     year = 1993,
    month = feb,
   volume = 403,
    pages = {L75-L78},
      doi = {10.1086/186725},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...403L..75C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{VandenBerg,
   author = {{VandenBerg}, D.~A. and {Richard}, O. and {Michaud}, G. and 
	{Richer}, J.},
    title = "{Models of Metal-poor Stars with Gravitational Settling and Radiative Accelerations. II. The Age of the Oldest Stars}",
  journal = {ApJ},
 keywords = {Convection, Diffusion, Galaxy: Globular Clusters: General, Stars: Abundances, Stars: Evolution, Stars: Population II},
     year = 2002,
    month = may,
   volume = 571,
    pages = {487-500},
      doi = {10.1086/339895},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...571..487V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Aguirre,
   author = {{Silva Aguirre}, V. and {Davies}, G.~R. and {Basu}, S. and {Christensen-Dalsgaard}, J. and 
	{Creevey}, O. and {Metcalfe}, T.~S. and {Bedding}, T.~R. and 
	{Casagrande}, L. and {Handberg}, R. and {Lund}, M.~N. and {Nissen}, P.~E. and 
	{Chaplin}, W.~J. and {Huber}, D. and {Serenelli}, A.~M. and 
	{Stello}, D. and {Van Eylen}, V. and {Campante}, T.~L. and {Elsworth}, Y. and 
	{Gilliland}, R.~L. and {Hekker}, S. and {Karoff}, C. and {Kawaler}, S.~D. and 
	{Kjeldsen}, H. and {Lundkvist}, M.~S.},
    title = "{Ages and fundamental properties of Kepler exoplanet host stars from asteroseismology}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1504.07992},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, planets and satellites: fundamental parameters, stars: evolution, stars: fundamental parameters, stars: oscillations, planetary systems},
     year = 2015,
    month = sep,
   volume = 452,
    pages = {2127-2148},
      doi = {10.1093/mnras/stv1388},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.452.2127S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Aguirre1,
   author = {{Silva Aguirre}, V. and {Lund}, M.~N. and {Antia}, H.~M. and 
	{Ball}, W.~H. and {Basu}, S. and {Christensen-Dalsgaard}, J. and 
	{Lebreton}, Y. and {Reese}, D.~R. and {Verma}, K. and {Casagrande}, L. and 
	{Justesen}, A.~B. and {Mosumgaard}, J.~R. and {Chaplin}, W.~J. and 
	{Bedding}, T.~R. and {Davies}, G.~R. and {Handberg}, R. and 
	{Houdek}, G. and {Huber}, D. and {Kjeldsen}, H. and {Latham}, D.~W. and 
	{White}, T.~R. and {Coelho}, H.~R. and {Miglio}, A. and {Rendle}, B.
	},
    title = "{Standing on the Shoulders of Dwarfs: the Kepler Asteroseismic LEGACY Sample. II.Radii, Masses, and Ages}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1611.08776},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: fundamental parameters, stars: oscillations},
     year = 2017,
    month = feb,
   volume = 835,
      eid = {173},
    pages = {173},
      doi = {10.3847/1538-4357/835/2/173},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...835..173S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Mathur,
   author = {{Mathur}, S. and {Metcalfe}, T.~S. and {Woitaszek}, M. and {Bruntt}, H. and 
	{Verner}, G.~A. and {Christensen-Dalsgaard}, J. and {Creevey}, O.~L. and 
	{Do{\v g}an}, G. and {Basu}, S. and {Karoff}, C. and {Stello}, D. and 
	{Appourchaux}, T. and {Campante}, T.~L. and {Chaplin}, W.~J. and 
	{Garc{\'{\i}}a}, R.~A. and {Bedding}, T.~R. and {Benomar}, O. and 
	{Bonanno}, A. and {Deheuvels}, S. and {Elsworth}, Y. and {Gaulme}, P. and 
	{Guzik}, J.~A. and {Handberg}, R. and {Hekker}, S. and {Herzberg}, W. and 
	{Monteiro}, M.~J.~P.~F.~G. and {Piau}, L. and {Quirion}, P.-O. and 
	{R{\'e}gulo}, C. and {Roth}, M. and {Salabert}, D. and {Serenelli}, A. and 
	{Thompson}, M.~J. and {Trampedach}, R. and {White}, T.~R. and 
	{Ballot}, J. and {Brand{\~a}o}, I.~M. and {Molenda-{\.Z}akowicz}, J. and 
	{Kjeldsen}, H. and {Twicken}, J.~D. and {Uddin}, K. and {Wohler}, B.
	},
    title = "{A Uniform Asteroseismic Analysis of 22 Solar-type Stars Observed by Kepler}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1202.2844},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, stars: evolution, stars: interiors, stars: oscillations},
     year = 2012,
    month = apr,
   volume = 749,
      eid = {152},
    pages = {152},
      doi = {10.1088/0004-637X/749/2/152},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...749..152M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Handberg,
   author = {{Handberg}, R. and {Lund}, M.~N.},
    title = "{Automated preparation of Kepler time series of planet hosts for asteroseismic analysis}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1409.1366},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, stars: oscillations, planetary systems},
     year = 2014,
    month = dec,
   volume = 445,
    pages = {2698-2709},
      doi = {10.1093/mnras/stu1823},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.445.2698H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lund,
   author = {{Lund}, M.~N. and {Silva Aguirre}, V. and {Davies}, G.~R. and 
	{Chaplin}, W.~J. and {Christensen-Dalsgaard}, J. and {Houdek}, G. and 
	{White}, T.~R. and {Bedding}, T.~R. and {Ball}, W.~H. and {Huber}, D. and 
	{Antia}, H.~M. and {Lebreton}, Y. and {Latham}, D.~W. and {Handberg}, R. and 
	{Verma}, K. and {Basu}, S. and {Casagrande}, L. and {Justesen}, A.~B. and 
	{Kjeldsen}, H. and {Mosumgaard}, J.~R.},
    title = "{Standing on the Shoulders of Dwarfs: the Kepler Asteroseismic LEGACY Sample. I. Oscillation Mode Parameters}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1612.00436},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: evolution, stars: fundamental parameters, stars: oscillations},
     year = 2017,
    month = feb,
   volume = 835,
      eid = {172},
    pages = {172},
      doi = {10.3847/1538-4357/835/2/172},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...835..172L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lebreton,
   author = {{Lebreton}, Y. and {Goupil}, M.~J.},
    title = "{Asteroseismology for ``{\`a} la carte'' stellar age-dating and weighing. Age and mass of the CoRoT exoplanet host HD 52265}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1406.0652},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: evolution, stars: fundamental parameters, planets and satellites: fundamental parameters, stars: individual: HD 52265, stars: interiors},
     year = 2014,
    month = sep,
   volume = 569,
      eid = {A21},
    pages = {A21},
      doi = {10.1051/0004-6361/201423797},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...569A..21L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Szentgyorgyi,
   author = {{Szentgyorgyi}, A.~H. and {Fur{\'e}sz}, G.},
    title = "{Precision Radial Velocities for the Kepler Era}",
 keywords = {Instrumentation: Spectrographs, Techniques: Radial Velocity, Stars: Planetary Systems: Protoplanetary disks},
booktitle = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
     year = 2007,
   series = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
   volume = 28,
   editor = {{Kurtz}, S.},
    month = jun,
    pages = {129-133},
   adsurl = {http://adsabs.harvard.edu/abs/2007RMxAC..28..129S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pinsonneault,
   author = {{Pinsonneault}, M.~H. and {An}, D. and {Molenda-{\.Z}akowicz}, J. and 
	{Chaplin}, W.~J. and {Metcalfe}, T.~S. and {Bruntt}, H.},
    title = "{A Revised Effective Temperature Scale for the Kepler Input Catalog}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1110.4456},
 primaryClass = "astro-ph.SR",
 keywords = {stars: fundamental parameters},
     year = 2012,
    month = apr,
   volume = 199,
      eid = {30},
    pages = {30},
      doi = {10.1088/0067-0049/199/2/30},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..199...30P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ram,
   author = {{Ram{\'{\i}}rez}, I. and {Mel{\'e}ndez}, J. and {Asplund}, M.
	},
    title = "{Accurate abundance patterns of solar twins and analogs. Does the anomalous solar chemical composition come from planet formation?}",
  journal = {A \& A},
 keywords = {stars: abundances, Sun: abundances, planetary systems},
     year = 2009,
    month = dec,
   volume = 508,
    pages = {L17-L20},
      doi = {10.1051/0004-6361/200913038},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...508L..17R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pinso,
   author = {{Pinsonneault}, M.~H. and {Elsworth}, Y. and {Epstein}, C. and 
	{Hekker}, S. and {M{\'e}sz{\'a}ros}, S. and {Chaplin}, W.~J. and 
	{Johnson}, J.~A. and {Garc{\'{\i}}a}, R.~A. and {Holtzman}, J. and 
	{Mathur}, S. and {Garc{\'{\i}}a P{\'e}rez}, A. and {Silva Aguirre}, V. and 
	{Girardi}, L. and {Basu}, S. and {Shetrone}, M. and {Stello}, D. and 
	{Allende Prieto}, C. and {An}, D. and {Beck}, P. and {Beers}, T.~C. and 
	{Bizyaev}, D. and {Bloemen}, S. and {Bovy}, J. and {Cunha}, K. and 
	{De Ridder}, J. and {Frinchaboy}, P.~M. and {Garc{\'{\i}}a-Hern{\'a}ndez}, D.~A. and 
	{Gilliland}, R. and {Harding}, P. and {Hearty}, F.~R. and {Huber}, D. and 
	{Ivans}, I. and {Kallinger}, T. and {Majewski}, S.~R. and {Metcalfe}, T.~S. and 
	{Miglio}, A. and {Mosser}, B. and {Muna}, D. and {Nidever}, D.~L. and 
	{Schneider}, D.~P. and {Serenelli}, A. and {Smith}, V.~V. and 
	{Tayar}, J. and {Zamora}, O. and {Zasowski}, G.},
    title = "{The APOKASC Catalog: An Asteroseismic and Spectroscopic Joint Survey of Targets in the Kepler Fields}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1410.2503},
 primaryClass = "astro-ph.SR",
 keywords = {catalogs, stars: abundances, stars: fundamental parameters, stars: oscillations: including pulsations, surveys},
     year = 2014,
    month = dec,
   volume = 215,
      eid = {19},
    pages = {19},
      doi = {10.1088/0067-0049/215/2/19},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..215...19P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pax1,
   author = {{Paxton}, B. and {Bildsten}, L. and {Dotter}, A. and {Herwig}, F. and 
	{Lesaffre}, P. and {Timmes}, F.},
    title = "{Modules for Experiments in Stellar Astrophysics (MESA)}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1009.1622},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, stars: evolution, stars: general},
     year = 2011,
    month = jan,
   volume = 192,
      eid = {3},
    pages = {3},
      doi = {10.1088/0067-0049/192/1/3},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..192....3P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pax2,
   author = {{Paxton}, B. and {Cantiello}, M. and {Arras}, P. and {Bildsten}, L. and 
	{Brown}, E.~F. and {Dotter}, A. and {Mankovich}, C. and {Montgomery}, M.~H. and 
	{Stello}, D. and {Timmes}, F.~X. and {Townsend}, R.},
    title = "{Modules for Experiments in Stellar Astrophysics (MESA): Planets, Oscillations, Rotation, and Massive Stars}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1301.0319},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, methods: numerical, planets and satellites: physical evolution, stars: evolution, stars: massive, stars: rotation},
     year = 2013,
    month = sep,
   volume = 208,
      eid = {4},
    pages = {4},
      doi = {10.1088/0067-0049/208/1/4},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..208....4P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Imbriani,
   author = {{Imbriani}, G. and {Costantini}, H. and {Formicola}, A. and 
	{Vomiero}, A. and {Angulo}, C. and {Bemmerer}, D. and {Bonetti}, R. and 
	{Broggini}, C. and {Confortola}, F. and {Corvisiero}, P. and 
	{Cruz}, J. and {Descouvemont}, P. and {F{\"u}l{\"o}p}, Z. and 
	{Gervino}, G. and {Guglielmetti}, A. and {Gustavino}, C. and 
	{Gy{\"u}rky}, G. and {Jesus}, A.~P. and {Junker}, M. and {Klug}, J.~N. and 
	{Lemut}, A. and {Menegazzo}, R. and {Prati}, P. and {Roca}, V. and 
	{Rolfs}, C. and {Romano}, M. and {Rossi-Alvarez}, C. and {Sch{\"u}mann}, F. and 
	{Sch{\"u}rmann}, D. and {Somorjai}, E. and {Straniero}, O. and 
	{Strieder}, F. and {Terrasi}, F. and {Trautvetter}, H.~P.},
    title = "{S-factor of $^{14}$N(p,{$\gamma$})$^{15}$O at astrophysical energies$^{⋆}$}",
  journal = {EPJ A},
   eprint = {nucl-ex/0509005},
 keywords = {25.40.Lw Radiative capture, 26.20.+f Hydrostatic stellar nucleosynthesis, 26.65.+t Solar neutrinos, 29.30.Kv X- and {$\gamma$}-ray spectroscopy},
     year = 2005,
    month = sep,
   volume = 25,
    pages = {455-466},
      doi = {10.1140/epja/i2005-10138-7},
   adsurl = {http://adsabs.harvard.edu/abs/2005EPJA...25..455I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Angulo,
   author = {{Angulo}, C. and {Arnould}, M. and {Rayet}, M. and {Descouvemont}, P. and 
	{Baye}, D. and {Leclercq-Willain}, C. and {Coc}, A. and {Barhoumi}, S. and 
	{Aguer}, P. and {Rolfs}, C. and {Kunz}, R. and {Hammer}, J.~W. and 
	{Mayer}, A. and {Paradellis}, T. and {Kossionides}, S. and {Chronidou}, C. and 
	{Spyrou}, K. and {degl'Innocenti}, S. and {Fiorentini}, G. and 
	{Ricci}, B. and {Zavatarelli}, S. and {Providencia}, C. and 
	{Wolters}, H. and {Soares}, J. and {Grama}, C. and {Rahighi}, J. and 
	{Shotter}, A. and {Lamehi Rachti}, M.},
    title = "{A compilation of charged-particle induced thermonuclear reaction rates}",
  journal = {Nuclear Physics A},
     year = 1999,
    month = aug,
   volume = 656,
    pages = {3-183},
      doi = {10.1016/S0375-9474(99)00030-5},
   adsurl = {http://adsabs.harvard.edu/abs/1999NuPhA.656....3A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sonoi,
   author = {{Sonoi}, T. and {Samadi}, R. and {Belkacem}, K. and {Ludwig}, H.-G. and 
	{Caffau}, E. and {Mosser}, B.},
    title = "{Surface-effect corrections for solar-like oscillations using 3D hydrodynamical simulations. I. Adiabatic oscillations}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1510.00300},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, convection, stars: atmospheres, stars: low-mass, stars: oscillations, stars: solar-type},
     year = 2015,
    month = nov,
   volume = 583,
      eid = {A112},
    pages = {A112},
      doi = {10.1051/0004-6361/201526838},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...583A.112S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Basu,
   author = {{Basu}, S. and {Antia}, H.~M.},
    title = "{Constraining Solar Abundances Using Helioseismology}",
  journal = {ApJL},
   eprint = {astro-ph/0403485},
 keywords = {Sun: Abundances, Sun: Interior, Sun: Oscillations},
     year = 2004,
    month = may,
   volume = 606,
    pages = {L85-L88},
      doi = {10.1086/421110},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...606L..85B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Scott,
   author = {{Scott}, P. and {Asplund}, M. and {Grevesse}, N. and {Bergemann}, M. and 
	{Sauval}, A.~J.},
    title = "{The elemental composition of the Sun. II. The iron group elements Sc to Ni}",
  journal = {A \ A },
archivePrefix = "arXiv",
   eprint = {1405.0287},
 primaryClass = "astro-ph.SR",
 keywords = {Sun: abundances, Sun: photosphere, Sun: granulation, line:, formation, line: profiles, convection},
     year = 2015,
    month = jan,
   volume = 573,
      eid = {A26},
    pages = {A26},
      doi = {10.1051/0004-6361/201424110},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...573A..26S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Grevesse2,
   author = {{Grevesse}, N. and {Scott}, P. and {Asplund}, M. and {Sauval}, A.~J.
	},
    title = "{The elemental composition of the Sun. III. The heavy elements Cu to Th}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1405.0288},
 primaryClass = "astro-ph.SR",
 keywords = {Sun: abundances, Sun: photosphere, Sun: granulation, line: formation, line: profiles, convection},
     year = 2015,
    month = jan,
   volume = 573,
      eid = {A27},
    pages = {A27},
      doi = {10.1051/0004-6361/201424111},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...573A..27G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ball,
   author = {{Ball}, W.~H. and {Gizon}, L.},
    title = "{A new correction of stellar oscillation frequencies for near-surface effects}",
  journal = {A \& A},
archivePrefix = "arXiv",
   eprint = {1408.0986},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, stars: oscillations, stars: individual: HD 52265},
     year = 2014,
    month = aug,
   volume = 568,
      eid = {A123},
    pages = {A123},
      doi = {10.1051/0004-6361/201424325},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...568A.123B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Townsend,
   author = {{Townsend}, R.~H.~D. and {Teitler}, S.~A.},
    title = "{GYRE: an open-source stellar oscillation code based on a new Magnus Multiple Shooting scheme}",
  journal = {MNRAS},
archivePrefix = "arXiv",
   eprint = {1308.2965},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, stars: evolution, stars: interiors, stars: oscillations, stars: variables: general},
     year = 2013,
    month = nov,
   volume = 435,
    pages = {3406-3418},
      doi = {10.1093/mnras/stt1533},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435.3406T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ferguson,
   author = {{Ferguson}, J.~W. and {Alexander}, D.~R. and {Allard}, F. and 
	{Barman}, T. and {Bodnarik}, J.~G. and {Hauschildt}, P.~H. and 
	{Heffner-Wong}, A. and {Tamanai}, A.},
    title = "{Low-Temperature Opacities}",
  journal = {ApJ},
   eprint = {astro-ph/0502045},
 keywords = {Atomic Data, Equation of State, Methods: Numerical, Molecular Data},
     year = 2005,
    month = apr,
   volume = 623,
    pages = {585-596},
      doi = {10.1086/428642},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...623..585F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cyburt,
   author = {{Cyburt}, R.~H. and {Fields}, B.~D. and {Olive}, K.~A.},
    title = "{Primordial nucleosynthesis in light of WMAP}",
  journal = {Physics Letters B},
   eprint = {astro-ph/0302431},
     year = 2003,
    month = aug,
   volume = 567,
    pages = {227-234},
      doi = {10.1016/j.physletb.2003.06.026},
   adsurl = {http://adsabs.harvard.edu/abs/2003PhLB..567..227C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kunz,
   author = {{Kunz}, R. and {Fey}, M. and {Jaeger}, M. and {Mayer}, A. and 
	{Hammer}, J.~W. and {Staudt}, G. and {Harissopulos}, S. and 
	{Paradellis}, T.},
    title = "{Astrophysical Reaction Rate of $^{12}$C({$\alpha$}, {$\gamma$})$^{16}$O}",
  journal = {ApJ},
 keywords = {Galaxy: Abundances, Nuclear Reactions, Nucleosynthesis, Abundances, Stars: Abundances, Stars: Evolution, Stars: Supernovae: General},
     year = 2002,
    month = mar,
   volume = 567,
    pages = {643-650},
      doi = {10.1086/338384},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...567..643K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Iglesias,
   author = {{Iglesias}, C.~A. and {Rogers}, F.~J.},
    title = "{Updated Opal Opacities}",
  journal = {ApJ},
 keywords = {ATOMIC DATA, ATOMIC PROCESSES, STARS: INTERIORS},
     year = 1996,
    month = jun,
   volume = 464,
    pages = {943},
      doi = {10.1086/177381},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...464..943I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rogers,
   author = {{Rogers}, F.~J. and {Nayfonov}, A.},
    title = "{Updated and Expanded OPAL Equation-of-State Tables: Implications for Helioseismology}",
  journal = {ApJ},
 keywords = {Atomic Processes, Equation of State, Sun: Oscillations},
     year = 2002,
    month = sep,
   volume = 576,
    pages = {1064-1074},
      doi = {10.1086/341894},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...576.1064R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vitense,
   author = {{B{\"o}hm-Vitense}, E.},
    title = "{{\"U}ber die Wasserstoffkonvektionszone in Sternen verschiedener Effektivtemperaturen und Leuchtkr{\"a}fte. Mit 5 Textabbildungen}",
  journal = {Zeit. Astrophys.},
     year = 1958,
   volume = 46,
    pages = {108},
   adsurl = {http://adsabs.harvard.edu/abs/1958ZA.....46..108B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pax3,
   author = {{Paxton}, B. and {Marchant}, P. and {Schwab}, J. and {Bauer}, E.~B. and 
	{Bildsten}, L. and {Cantiello}, M. and {Dessart}, L. and {Farmer}, R. and 
	{Hu}, H. and {Langer}, N. and {Townsend}, R.~H.~D. and {Townsley}, D.~M. and 
	{Timmes}, F.~X.},
    title = "{Modules for Experiments in Stellar Astrophysics (MESA): Binaries, Pulsations, and Explosions}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1506.03146},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: general, methods: numerical, nuclear reactions, nucleosynthesis, abundances, shock waves, stars: evolution, stars: oscillations},
     year = 2015,
    month = sep,
   volume = 220,
      eid = {15},
    pages = {15},
      doi = {10.1088/0067-0049/220/1/15},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJS..220...15P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Casa,
   author = {{Casagrande}, L. and {Silva Aguirre}, V. and {Stello}, D. and 
	{Huber}, D. and {Serenelli}, A.~M. and {Cassisi}, S. and {Dotter}, A. and 
	{Milone}, A.~P. and {Hodgkin}, S. and {Marino}, A.~F. and {Lund}, M.~N. and 
	{Pietrinferni}, A. and {Asplund}, M. and {Feltzing}, S. and 
	{Flynn}, C. and {Grundahl}, F. and {Nissen}, P.~E. and {Sch{\"o}nrich}, R. and 
	{Schlesinger}, K.~J. and {Wang}, W.},
    title = "{Str{\"o}mgren Survey for Asteroseismology and Galactic Archaeology: Let the SAGA Begin}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1403.2754},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy: stellar content, stars: abundances, stars: distances, stars: fundamental parameters, stars: oscillations, surveys, techniques: photometric},
     year = 2014,
    month = jun,
   volume = 787,
      eid = {110},
    pages = {110},
      doi = {10.1088/0004-637X/787/2/110},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...787..110C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Buchhave,
   author = {{Buchhave}, L.~A. and {Latham}, D.~W. and {Johansen}, A. and 
	{Bizzarro}, M. and {Torres}, G. and {Rowe}, J.~F. and {Batalha}, N.~M. and 
	{Borucki}, W.~J. and {Brugamyer}, E. and {Caldwell}, C. and 
	{Bryson}, S.~T. and {Ciardi}, D.~R. and {Cochran}, W.~D. and 
	{Endl}, M. and {Esquerdo}, G.~A. and {Ford}, E.~B. and {Geary}, J.~C. and 
	{Gilliland}, R.~L. and {Hansen}, T. and {Isaacson}, H. and {Laird}, J.~B. and 
	{Lucas}, P.~W. and {Marcy}, G.~W. and {Morse}, J.~A. and {Robertson}, P. and 
	{Shporer}, A. and {Stefanik}, R.~P. and {Still}, M. and {Quinn}, S.~N.
	},
    title = "{An abundance of small exoplanets around stars with a wide range of metallicities}",
  journal = {Nature},
     year = 2012,
    month = jun,
   volume = 486,
    pages = {375-377},
      doi = {10.1038/nature11121},
   adsurl = {http://adsabs.harvard.edu/abs/2012Natur.486..375B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kjeldsen,
   author = {{Kjeldsen}, H. and {Bedding}, T.~R. and {Butler}, R.~P. and 
	{Christensen-Dalsgaard}, J. and {Kiss}, L.~L. and {McCarthy}, C. and 
	{Marcy}, G.~W. and {Tinney}, C.~G. and {Wright}, J.~T.},
    title = "{Solar-like Oscillations in {$\alpha$} Centauri B}",
  journal = {ApJ},
   eprint = {astro-ph/0508609},
 keywords = {Stars: Individual: Constellation Name: {$\alpha$} Centauri A, Stars: Individual: Constellation Name: {$\alpha$} Centauri B, Stars: Individual: Constellation Name: {$\beta$} Hydri, stars: individual ({$\delta$} Pavonis), Stars: Oscillations, Sun: Helioseismology},
     year = 2005,
    month = dec,
   volume = 635,
    pages = {1281-1290},
      doi = {10.1086/497530},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...635.1281K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kjeldsen1,
   author = {{Kjeldsen}, H. and {Bedding}, T.~R.},
    title = "{Amplitudes of stellar oscillations: the implications for asteroseismology.}",
  journal = {A \& A},
   eprint = {astro-ph/9403015},
 keywords = {SUN: OSCILLATIONS, STARS: INDIVIDUAL: $\{$ALPHA$\}$ CEN, STARS: INDIVIDUAL: PROCYON, STARS: OSCILLATIONS, CEPHEIDS, $\{$DELTA$\}$ SCT},
     year = 1995,
    month = jan,
   volume = 293,
    pages = {87-106},
   adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...293...87K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Foreman,
   author = {{Foreman-Mackey}, D. and {Hogg}, D.~W. and {Lang}, D. and {Goodman}, J.
	},
    title = "{emcee: The MCMC Hammer}",
  journal = {PASP},
archivePrefix = "arXiv",
   eprint = {1202.3665},
 primaryClass = "astro-ph.IM",
     year = 2013,
    month = mar,
   volume = 125,
    pages = {306},
      doi = {10.1086/670067},
   adsurl = {http://adsabs.harvard.edu/abs/2013PASP..125..306F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




